Data-Driven Active Power Flow Modeling: A Behavioral Systems Approach

The increasing decentralization of power systems driven by a large number of renewable energy sources poses challenges in power flow optimization: Partially unknown power line properties can render model-based approaches unsuitable. With the increasing deployment of sensors, data-driven methods rise as a promising alternative, offering flexibility to adapt changes and deal with unknown properties. In this paper, we propose a novel data-driven representation of nonlinear active power flow equations for radial grids based on Willems' Fundamental Lemma. Our approach allows for direct integration of input/output data into active power flow optimization, enabling cost minimization and constraint enforcement without requiring explicit knowledge of the electrical properties of the grid. Moreover, we derive a computationally tractable convex relaxation and show in a numerical case study that our approaches yield results that are identical to optimal active power flow formulations with known parameters.

==> figures/NewNodeCommands.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US
% !TEX TS-program = pdflatex
% !TEX root = ../slides.tex

\newcommand{\lnwidth}{0.6pt}
% \newcommand{\lngrid}{0.5pt}
\newcommand{\scaleSymbols}{0.04}

\newcommand{\GraphLine}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter,line cap=round,miter limit=4.00,rounded corners=0.0000cm] (0,0)
	rectangle (24,1);
	\path[draw] (7, 0.5) -- (17, 0.5);
	\end{tikzpicture}}

\newcommand{\GraphLineFlip}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, rotate=90]
	\path[line join=miter,line cap=round,miter limit=4.00, rounded corners=0.0000cm] (0,0)
	rectangle (24,1);
	\path[draw] (7, 0.5) -- (17, 0.5);
	\end{tikzpicture}}

\newcommand{\GraphTransformer}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter,line cap=round,miter limit=4.00, rounded corners=0.0000cm] (0,0)
	rectangle (24,24);
	\path[draw=none, fill=white] (12, 15) circle (6);
	\path[draw, fill=white] (12, 9) circle (6);
	\path[draw] (12, 15) circle (6);
	\end{tikzpicture}}

\newcommand{\GraphTransformerFlip}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, rotate=90]
	\path[line join=miter,line cap=round,miter limit=4.00, rounded corners=0.0000cm] (0,0)
	rectangle (24,24);
	\path[draw=none, fill=white] (12, 15) circle (6);
	\path[draw, fill=white] (12, 9) circle (6);
	\path[draw] (12, 15) circle (6);
	\end{tikzpicture}}

\newcommand{\GraphInverter}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
	\path[line join=miter, line cap=round, miter limit=4.00, line width=\lnwidth,
			rounded corners=0.0000cm] (0,0) rectangle (24,24);
	\path[draw, line join=miter, line cap=butt, miter limit=4.00, line width=\lnwidth] (22, 2) -- (2, 22);
	\draw [line width=\lnwidth] plot [smooth, tension=1] coordinates { (21, 19) (18, 16) (15, 19) (12, 16)};
	\draw [line width=\lnwidth]
		(4, 5.25) -- (11, 5.25)
		(4, 7.75) -- (11, 7.75);
	\end{tikzpicture}}

\newcommand{\GraphInverterFlip}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
	\path[line join=miter, line cap=round, miter limit=4.00, line width=\lnwidth,
	rounded corners=0.0000cm] (0,0) rectangle (24,24);
	\path[draw, line join=miter, line cap=butt, miter limit=4.00, line width=\lnwidth] (22, 2) -- (2, 22);
	\draw [line width=\lnwidth] plot [smooth, tension=1] coordinates { (21, 19) (18, 16) (15, 19) (12, 16)};
	\draw [line width=\lnwidth]
	(4, 5.25) -- (11, 5.25)
	(4, 7.75) -- (11, 7.75);
	\end{tikzpicture}}

\newcommand{\tower}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
         limit=4.00,line width=\lnwidth,rounded corners=0.0000cm]
				(0,0)
       rectangle (24,24);
   \draw (-1,0) arc (180:360:1cm and 0.5cm);
    \draw (-1,0) arc (180:0:1cm and 0.5cm);
    \draw (-2,-3) arc (180:360:2cm and 1cm);
    %\draw[dashed] (-2,-3) arc (180:10:2cm and 1cm);
    \draw(-2,-3)  -- (-1,0);
    \draw(2,-3)   -- (1,0);
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (-1,0) arc (180:360:1cm and 0.5cm) -- (2,-3) arc (360:180:2cm and 1cm) -- cycle;
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (0,0) circle (1cm and 0.5cm);
\end{tikzpicture}
}

\newcommand{\GraphTristateTF}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (4,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (20,12) -- (24,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) circle (5);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (9,12) circle (5);
\end{tikzpicture}}

\newcommand{\GraphTristatePCC}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (9,12) -- (15,6);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) -- (24,12);
\end{tikzpicture}}

\newcommand{\GraphTristateR}{
%	\renewcommand{\linewidthR}m}
\begin{tikzpicture}[scale = \scaleSymbols, >=latex, color=black]
        \path[] (315.0000,52.3622-1) rectangle (335.0000,72.3622-1);
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=1.5*\lnwidth] (324.0306,59.8874) .. controls (321.9302,58.2551) and
          (319.7014,56.9114) .. (317.2333,55.6929) .. controls (319.8093,57.9660) and
          (324.1469,60.6035) .. (324.0306,59.8874) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=1.5*\lnwidth] (325.5865,60.4167) .. controls (328.0392,59.6017) and
          (330.4240,58.6404) .. (332.7667,57.0558) .. controls (329.8032,57.9971) and
          (326.8503,59.6115) .. (325.5865,60.4167) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=1.5*\lnwidth] (324.8607,61.1176) .. controls (324.6795,63.5961) and
          (324.6662,66.1651) .. (325.3315,69.0315) .. controls (325.5549,66.1044) and
          (325.1090,62.6873) .. (324.8607,61.1176) -- cycle;
        \path[cm={{0.20207,0.0904,-0.09626,0.21517,(296.36236,26.26027)}},draw,fill,line
          join=round,line cap=round,miter limit=4.00,line width=2*\lnwidth]
          (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
          (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
          (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
          (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
          (186.0000,84.3622) -- cycle;
\end{tikzpicture}
}

%===================

\newcommand{\GraphTristateS}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (265.0000,52.3622)
          rectangle (285.0000,72.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (269.0000,61.3622) -- (281.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,55.3622) -- (275.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (272.0000,63.3622) -- (278.0000,63.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,63.3622) -- (275.0000,69.3622);
\end{tikzpicture}
}


% %===================

\newcommand{\GraphTristateT}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622-.5)
          rectangle (515.0000,72.3622-.5);
        \path[cm={{0.38462,0.0,0.0,0.83333,(380.9615,-59.27301)}},draw, line
          join=round,line cap=round,miter limit=4.00,line width=\lnwidth, color = black]
          (342.0000,145.3622) .. controls (342.0000,150.3328) and (333.2695,154.3622) ..
          (322.5000,154.3622) .. controls (311.7305,154.3622) and (303.0000,150.3328) ..
          (303.0000,145.3622) .. controls (303.0000,140.3916) and (311.7305,136.3622) ..
          (322.5000,136.3622) .. controls (333.2695,136.3622) and (342.0000,140.3916) ..
          (342.0000,145.3622) -- cycle;
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth, color = black]
          (505.0000,54.3622) -- (505.0000,69.3622);
\end{tikzpicture}
}


% %===================

\newcommand{\GraphTristateP}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622)
          rectangle node {N} (515.0000,72.3622) ;
\end{tikzpicture}
}

% %===================

\newcommand{\GraphTristatePV}{
\begin{tikzpicture}[scale =  -\scaleSymbols, >=latex, color=black]
%=== PV ===
  \begin{scope}[cm={{1.33333,0.0,0.0,1.33333,(-219.66665,-77.45405)}}]
    \path[line join=miter,line cap=round,miter
      limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (371.0000,157.3622)
      rectangle (386.0000,172.3622);
    \begin{scope}[cm={{0.75,0.0,0.0,0.75,(108.84792,54.02778)}}]
      \path[cm={{0.45455,0.21485,-0.21652,0.51139,(295.25671,66.03768)}},draw=white,fill,line
        join=round,line cap=round,miter limit=4.00,line width=1*\lnwidth]
        (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
        (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
        (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
        (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
        (186.0000,84.3622) -- cycle;
      \begin{scope}[shift={(-0.46388,0.41703)}]
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.2097,144.9631) -- (368.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,151.3622) -- (356.4103,149.0251);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.3146,147.2675) -- (368.0000,147.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,143.3622) -- (356.1804,145.6575);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (368.0000,155.3622) -- (362.5254,149.6350);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (358.2954,144.1423) -- (356.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (360.0000,155.3622) -- (359.9369,151.0555);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,155.3622) -- (357.0000,150.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,147.3622) -- (356.2119,147.4569);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,139.3622) -- (357.1274,144.7105);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (359.8422,144.3002) -- (360.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (361.3258,144.2370) -- (364.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (356.0000,155.3622) -- (358.2954,150.8977);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.6832,145.9732) -- (368.0000,142.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.2514,148.3092) -- (368.0000,149.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (364.6693,154.2802) -- (361.4307,150.5189);
      \end{scope}
    \end{scope}
  \end{scope}
\end{tikzpicture}
}

